FocusedCleaner: Sanitizing Poisoned Graphs for Robust GNN-based Node Classification

Graph Neural Networks (GNNs) are vulnerable to data poisoning attacks, which will generate a poisoned graph as the input to the GNN models. We present FocusedCleaner as a poisoned graph sanitizer to effectively identify the poison injected by attackers. Specifically, FocusedCleaner provides a sanitation framework consisting of two modules: bi-level structural learning and victim node detection. In particular, the structural learning module will reverse the attack process to steadily sanitize the graph while the detection module provides ``the focus" -- a narrowed and more accurate search region -- to structural learning. These two modules will operate in iterations and reinforce each other to sanitize a poisoned graph step by step. As an important application, we show that the adversarial robustness of GNNs trained over the sanitized graph for the node classification task is significantly improved. Extensive experiments demonstrate that FocusedCleaner outperforms the state-of-the-art baselines both on poisoned graph sanitation and improving robustness.

==> citation.tex <==
@inproceedings{
	gcn,
	title={Semi-Supervised Classification with Graph Convolutional Networks},
	author={Thomas N. Kipf and Max Welling},
	booktitle={International Conference on Learning Representations},
	year={2017},
	url={https://openreview.net/forum?id=SJU4ayYgl}
}

@article{citationgraph,
  title={Automating the construction of internet portals with machine learning},
  author={McCallum, Andrew Kachites and Nigam, Kamal and Rennie, Jason and Seymore, Kristie},
  journal={Information Retrieval},
  volume={3},
  pages={127--163},
  year={2000},
  publisher={Springer}
}

@article{sen2008collective,
  title={Collective classification in network data},
  author={Sen, Prithviraj and Namata, Galileo and Bilgic, Mustafa and Getoor, Lise and Galligher, Brian and Eliassi-Rad, Tina},
  journal={AI magazine},
  volume={29},
  number={3},
  pages={93--93},
  year={2008}
}

@article{GADsurvey,
  title={A comprehensive survey on graph anomaly detection with deep learning},
  author={Ma, Xiaoxiao and Wu, Jia and Xue, Shan and Yang, Jian and Zhou, Chuan and Sheng, Quan Z and Xiong, Hui and Akoglu, Leman},
  journal={IEEE Transactions on Knowledge and Data Engineering},
  year={2021},
  publisher={IEEE}
}

@inproceedings{GIN,
title={How Powerful are Graph Neural Networks?},
author={Keyulu Xu and Weihua Hu and Jure Leskovec and Stefanie Jegelka},
booktitle={International Conference on Learning Representations},
year={2019},
url={https://openreview.net/forum?id=ryGs6iA5Km},
}

@inproceedings{
	mettack,
	title={Adversarial Attacks on Graph Neural Networks via Meta Learning},
	author={Daniel Zügner and Stephan Günnemann},
	booktitle={International Conference on Learning Representations},
	year={2019},
	url={https://openreview.net/forum?id=Bylnx209YX},
}

@book{entropy,
  title={The theory of information and coding},
  author={McEliece, Robert},
  volume={3},
  year={2002},
  publisher={Cambridge University Press}
}

@article {jaccardidx,
      author = "Allan H.  Murphy",
      title = "The Finley Affair: A Signal Event in the History of Forecast Verification",
      journal = "Weather and Forecasting",
      year = "1996",
      publisher = "American Meteorological Society",
      address = "Boston MA, USA",
      volume = "11",
      number = "1",
      doi = "10.1175/1520-0434(1996)011<0003:TFAASE>2.0.CO;2",
      pages=      "3 - 20",
      url = "https://journals.ametsoc.org/view/journals/wefo/11/1/1520-0434_1996_011_0003_tfaase_2_0_co_2.xml"
}

@article{poison,
  title={Detection of adversarial training examples in poisoning attacks through anomaly detection},
  author={Paudice, Andrea and Mu{\~n}oz-Gonz{\'a}lez, Luis and Gyorgy, Andras and Lupu, Emil C},
  journal={arXiv preprint arXiv:1802.03041},
  year={2018}
}

@article{RS,
  title={Recommender systems survey},
  author={Bobadilla, Jes{\'u}s and Ortega, Fernando and Hernando, Antonio and Guti{\'e}rrez, Abraham},
  journal={Knowledge-based systems},
  volume={46},
  pages={109--132},
  year={2013},
  publisher={Elsevier}
}

@inproceedings{topologyattack,
author = {Xu, Kaidi and Chen, Hongge and Liu, Sijia and Chen, Pin-Yu and Weng, Tsui-Wei and Hong, Mingyi and Lin, Xue},
title = {Topology Attack and Defense for Graph Neural Networks: An Optimization Perspective},
year = {2019},
isbn = {9780999241141},
publisher = {AAAI Press},
abstract = {Graph neural networks (GNNs) which apply the deep neural networks to graph data have achieved significant performance for the task of semi-supervised node classification. However, only few work has addressed the adversarial robustness of GNNs. In this paper, we first present a novel gradient-based attack method that facilitates the difficulty of tackling discrete graph data. When comparing to current adversarial attacks on GNNs, the results show that by only perturbing a small number of edge perturbations, including addition and deletion, our optimization-based attack can lead to a noticeable decrease in classification performance. Moreover, leveraging our gradient-based attack, we propose the first optimization-based adversarial training for GNNs. Our method yields higher robustness against both different gradient based and greedy attack methods without sacrificing classification accuracy on original graph.},
booktitle = {Proceedings of the 28th International Joint Conference on Artificial Intelligence},
pages = {3961–3967},
numpages = {7},
location = {Macao, China},
series = {IJCAI'19}
}

@inproceedings{GNNGUARD,
	title     = {GNNGuard: Defending Graph Neural Networks against Adversarial Attacks},
	author    = {Zhang, Xiang and Zitnik, Marinka},
	booktitle = {Proceedings of Neural Information Processing Systems, NeurIPS},
	year      = {2020}
}

@inproceedings{attackCD,
	title={Adversarial attack on community detection by hiding individuals},
	author={Li, Jia and Zhang, Honglei and Han, Zhichao and Rong, Yu and Cheng, Hong and Huang, Junzhou},
	booktitle={Proceedings of The Web Conference 2020},
	pages={917--927},
	year={2020}
}

@inproceedings{RGCN,
	title={Robust graph convolutional networks against adversarial attacks},
	author={Zhu, Dingyuan and Zhang, Ziwei and Cui, Peng and Zhu, Wenwu},
	booktitle={Proceedings of the 25th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
	pages={1399--1407},
	year={2019}
}

@inproceedings{ProGNN,
	title={Graph structure learning for robust graph neural networks},
	author={Jin, Wei and Ma, Yao and Liu, Xiaorui and Tang, Xianfeng and Wang, Suhang and Tang, Jiliang},
	booktitle={Proceedings of the 26th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
	pages={66--74},
	year={2020}
}

@article{relu,
	title={Deep learning using rectified linear units (relu)},
	author={Agarap, Abien Fred},
	journal={arXiv preprint arXiv:1803.08375},
	year={2018}
}

@inproceedings{adam,
	author    = {Diederik P. Kingma and
	Jimmy Ba},
	editor    = {Yoshua Bengio and
	Yann LeCun},
	title     = {Adam: {A} Method for Stochastic Optimization},
	booktitle = {3rd International Conference on Learning Representations, {ICLR} 2015,
	San Diego, CA, USA, May 7-9, 2015, Conference Track Proceedings},
	year      = {2015},
	url       = {http://arxiv.org/abs/1412.6980},
	timestamp = {Thu, 25 Jul 2019 14:25:37 +0200},
	biburl    = {https://dblp.org/rec/journals/corr/KingmaB14.bib},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{attackLP,
	author = {Lin, Wanyu and Ji, Shengxiang and Li, Baochun},
	title = {Adversarial Attacks on Link Prediction Algorithms Based on Graph Neural Networks},
	year = {2020},
	isbn = {9781450367509},
	publisher = {Association for Computing Machinery},
	address = {New York, NY, USA},
	url = {https://doi.org/10.1145/3320269.3384750},
	doi = {10.1145/3320269.3384750},
	abstract = {Link prediction is one of the fundamental problems for graph-structured data. However, a number of applications of link prediction, such as predicting commercial ties or memberships within a criminal organization, are adversarial, with another party aiming to minimize its effectiveness by manipulating observed information about the graph. In this paper, we focus on the feasibility of mounting adversarial attacks against link prediction algorithms based on graph neural networks. We first propose a greedy heuristic that exploits incremental computation to find attacks against a state-of-the-art link prediction algorithm, called SEAL. We then design an efficient variant of this algorithm that incorporates the link formation mechanism and Υ-decaying heuristic theory to design more effective adversarial attacks. We used real-world datasets and performed an extensive array of experiments to show that the performance of SEAL is negatively affected by a significant margin. More importantly, our experimental results have shown that our adversarial attacks mounted based on SEAL can be readily transferred to several existing link prediction heuristics in the literature.},
	booktitle = {Proceedings of the 15th ACM Asia Conference on Computer and Communications Security},
	pages = {370–380},
	numpages = {11},
	keywords = {adversarial attacks, graph neural networks, link prediction},
	location = {Taipei, Taiwan},
	series = {ASIA CCS '20}
}

@inproceedings{expressive,
  title={Expressive 1-lipschitz neural networks for robust multiple graph learning against adversarial attacks},
  author={Zhao, Xin and Zhang, Zeru and Zhang, Zijie and Wu, Lingfei and Jin, Jiayin and Zhou, Yang and Jin, Ruoming and Dou, Dejing and Yan, Da},
  booktitle={International Conference on Machine Learning},
  pages={12719--12735},
  year={2021},
  organization={PMLR}
}

@INPROCEEDINGS{attackLPsimilarity,
  author={Zhou, Kai and Michalak, Tomasz P. and Vorobeychik, Yevgeniy},
  booktitle={2019 IEEE International Conference on Data Mining (ICDM)}, 
  title={Adversarial Robustness of Similarity-Based Link Prediction}, 
  year={2019},
  volume={},
  number={},
  pages={926-935},
  doi={10.1109/ICDM.2019.00103}}

@inproceedings{graphattack,
  title={Adversarial attack on graph structured data},
  author={Dai, Hanjun and Li, Hui and Tian, Tian and Huang, Xin and Wang, Lin and Zhu, Jun and Song, Le},
  booktitle={International conference on machine learning},
  pages={1115--1124},
  year={2018},
  organization={PMLR}
}

@inproceedings{graphbackdoor,
  title={Graph backdoor},
  author={Xi, Zhaohan and Pang, Ren and Ji, Shouling and Wang, Ting},
  booktitle={30th USENIX Security Symposium (USENIX Security 21)},
  pages={1523--1540},
  year={2021}
}

@INPROCEEDINGS{graphsac,
  author={Ioannidis, Vassilis N. and Berberidis, Dimitris and Giannakis, Georgios B.},
  booktitle={ICASSP 2021 - 2021 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)}, 
  title={Unveiling Anomalous Nodes Via Random Sampling and Consensus on Graphs}, 
  year={2021},
  volume={},
  number={},
  pages={5499-5503},
  doi={10.1109/ICASSP39728.2021.9414953}}

@inproceedings{aane,
  title={AANE: Anomaly aware network embedding for anomalous link detection},
  author={Duan, Dongsheng and Tong, Lingling and Li, Yangxi and Lu, Jie and Shi, Lei and Zhang, Cheng},
  booktitle={2020 IEEE International Conference on Data Mining (ICDM)},
  pages={1002--1007},
  year={2020},
  organization={IEEE}
}

@article{MultiscaleEP,
  title={Multiscale Evolutionary Perturbation Attack on Community Detection},
  author={Jinyin Chen and Yixian Chen and Lihong Chen and M. Zhao and Qi Xuan},
  journal={IEEE Transactions on Computational Social Systems},
  year={2021},
  volume={8},
  pages={62-75}
}

@inproceedings{prox12,
  title={Comparing and detecting adversarial attacks for graph deep learning},
  author={Zhang, Yingxue and Khan, S and Coates, Mark},
  booktitle={Proc. Representation Learning on Graphs and Manifolds Workshop, Int. Conf. Learning Representations, New Orleans, LA, USA},
  year={2019}
}

@article{Gmean,
  title={Machine learning for the detection of oil spills in satellite radar images},
  author={Kubat, Miroslav and Holte, Robert C and Matwin, Stan},
  journal={Machine learning},
  volume={30},
  number={2},
  pages={195--215},
  year={1998},
  publisher={Springer}
}

@book{mlp,
  title={Neural networks: a comprehensive foundation},
  author={Haykin, Simon},
  year={1994},
  publisher={Prentice Hall PTR}
}

@article{PCA,
author = { Karl   Pearson   F.R.S. },
title = {LIII. On lines and planes of closest fit to systems of points in space},
journal = {The London, Edinburgh, and Dublin Philosophical Magazine and Journal of Science},
volume = {2},
number = {11},
pages = {559-572},
year  = {1901},
publisher = {Taylor & Francis},
doi = {10.1080/14786440109462720},
}

@inproceedings{
DGMM,
title={Deep Autoencoding Gaussian Mixture Model for Unsupervised Anomaly Detection},
author={Bo Zong and Qi Song and Martin Renqiang Min and Wei Cheng and Cristian Lumezanu and Daeki Cho and Haifeng Chen},
booktitle={International Conference on Learning Representations},
year={2018},
url={https://openreview.net/forum?id=BJJLHbb0-},
}

@article{KL,
author = {I. Csiszar},
title = {{$I$-Divergence Geometry of Probability Distributions and Minimization Problems}},
volume = {3},
journal = {The Annals of Probability},
number = {1},
publisher = {Institute of Mathematical Statistics},
pages = {146 -- 158},
keywords = {15-A48, 49-F22, 60-00-E05, 62-B10, Contingency tables, distributions with given marginals, Geometry of probability distributions, iterative proportional fitting procedure, minimum discrimination information},
year = {1975},
doi = {10.1214/aop/1176996454},
URL = {https://doi.org/10.1214/aop/1176996454}
}

@inproceedings{egonetwork,
  title={Predicting defects using network analysis on dependency graphs},
  author={Zimmermann, Thomas and Nagappan, Nachiappan},
  booktitle={Proceedings of the 30th international conference on Software engineering},
  pages={531--540},
  year={2008}
}

@inproceedings{jsdiv,
  title={Detection and defense of topological adversarial attacks on graphs},
  author={Zhang, Yingxue and Regol, Florence and Pal, Soumyasundar and Khan, Sakif and Ma, Liheng and Coates, Mark},
  booktitle={International Conference on Artificial Intelligence and Statistics},
  pages={2989--2997},
  year={2021},
  organization={PMLR}
}

@inproceedings{attackLPsim2,
title = "Attacking similarity-based link prediction in social networks",
keywords = "Adversarial attacks, Computational social science, Link prediction, Security and privacy",
author = "Kai Zhou and Michalak, {Tomasz P.} and Marcin Waniek and Talal Rahwan and Yevgeniy Vorobeychik",
year = "2019",
language = "English",
series = "Proceedings of the International Joint Conference on Autonomous Agents and Multiagent Systems, AAMAS",
pages = "305--313",
booktitle = "18th International Conference on Autonomous Agents and Multiagent Systems, AAMAS 2019",
}

@book{PGD,
  title={Convex analysis},
  author={Rockafellar, R Tyrrell},
  volume={11},
  year={1997},
  publisher={Princeton university press}
}

@INPROCEEDINGS{binarizedattack,
	author={Zhu, Yulin and Lai, Yuni and Zhao, Kaifa and Luo, Xiapu and Yuan, Mingquan and Ren, Jian and Zhou, Kai},
	booktitle={2022 IEEE 38th International Conference on Data Engineering (ICDE)}, 
	title={BinarizedAttack: Structural Poisoning Attacks to Graph-based Anomaly Detection}, 
	year={2022},
	volume={},
	number={},
	pages={14-26},
	doi={10.1109/ICDE53745.2022.00006}}

@article{greatx,
	title={Recent advances in reliable deep graph learning: Adversarial attack, inherent noise, and distribution shift},
	author={Wu, Bingzhe and Li, Jintang and Hou, Chengbin and Fu, Guoji and Bian, Yatao and Chen, Liang and Huang, Junzhou},
	journal={arXiv preprint arXiv:2202.07114},
	year={2022}
}

@article{graphsage,
  title={Inductive representation learning on large graphs},
  author={Hamilton, Will and Ying, Zhitao and Leskovec, Jure},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}

@inproceedings{mediangnn,
  title     = {Understanding Structural Vulnerability in Graph Convolutional Networks},
  author    = {Chen, Liang and Li, Jintang and Peng, Qibiao and Liu, Yang and Zheng, Zibin and Yang, Carl},
  booktitle = {Proceedings of the Thirtieth International Joint Conference on
               Artificial Intelligence, {IJCAI-21}},
  publisher = {International Joint Conferences on Artificial Intelligence Organization},
  editor    = {Zhi-Hua Zhou},
  pages     = {2249--2255},
  year      = {2021},
  month     = {8},
  note      = {Main Track},
  doi       = {10.24963/ijcai.2021/310},
  url       = {https://doi.org/10.24963/ijcai.2021/310},
}

@inproceedings{elasticgnn,
	title={Elastic graph neural networks},
	author={Liu, Xiaorui and Jin, Wei and Ma, Yao and Li, Yaxin and Liu, Hua and Wang, Yiqi and Yan, Ming and Tang, Jiliang},
	booktitle={International Conference on Machine Learning},
	pages={6837--6849},
	year={2021},
	organization={PMLR}
}

@inproceedings{simpgcn,
	title={Node similarity preserving graph convolutional networks},
	author={Jin, Wei and Derr, Tyler and Wang, Yiqi and Ma, Yao and Liu, Zitao and Tang, Jiliang},
	booktitle={Proceedings of the 14th ACM international conference on web search and data mining},
	pages={148--156},
	year={2021}
}

@article{airgnn,
	title={Graph neural networks with adaptive residual},
	author={Liu, Xiaorui and Ding, Jiayuan and Jin, Wei and Xu, Han and Ma, Yao and Liu, Zitao and Tang, Jiliang},
	journal={Advances in Neural Information Processing Systems},
	volume={34},
	pages={9720--9733},
	year={2021}
}

@inproceedings{gcnjaccard,
	title     = {Adversarial Examples for Graph Data: Deep Insights into Attack and Defense},
	author    = {Wu, Huijun and Wang, Chen and Tyshetskiy, Yuriy and Docherty, Andrew and Lu, Kai and Zhu, Liming},
	booktitle = {Proceedings of the Twenty-Eighth International Joint Conference on
	Artificial Intelligence, {IJCAI-19}},
	publisher = {International Joint Conferences on Artificial Intelligence Organization},
	pages     = {4816--4823},
	year      = {2019},
	month     = {7},
	doi       = {10.24963/ijcai.2019/669},
	url       = {https://doi.org/10.24963/ijcai.2019/669},
}

@book{LCC,
  title={A First Look at Graph Theory},
  author={Clark, J. and Holton, D.A.},
  isbn={9789810204907},
  lccn={91014633},
  url={https://books.google.com.hk/books?id=vLRNRebXuKYC},
  year={1991},
  publisher={World Scientific}
}

@inproceedings{maskGVAE,
	title={Mask-GVAE: Blind Denoising Graphs via Partition},
	author={Li, Jia and Liu, Mengzhou and Zhang, Honglei and Wang, Pengyun and Wen, Yong and Pan, Lujia and Cheng, Hong},
	booktitle={Proceedings of the ACM Web Conference 2021},
	pages={3688–3698},
	year={2021}
}

@inproceedings{GASOLINE,
	title={Graph sanitation with application to node classification},
	author={Xu, Zhe and Du, Boxin and Tong, Hanghang},
	booktitle={Proceedings of the ACM Web Conference 2022},
	pages={1136--1147},
	year={2022}
}

@article{momentum,
  title={On the momentum term in gradient descent learning algorithms},
  author={Qian, Ning},
  journal={Neural networks},
  volume={12},
  number={1},
  pages={145--151},
  year={1999},
  publisher={Elsevier}
}

@article{survey,
	author = {Jin, Wei and Li, Yaxing and Xu, Han and Wang, Yiqi and Ji, Shuiwang and Aggarwal, Charu and Tang, Jiliang},
	title = {Adversarial Attacks and Defenses on Graphs},
	year = {2021},
	issue_date = {December 2020},
	publisher = {Association for Computing Machinery},
	address = {New York, NY, USA},
	volume = {22},
	number = {2},
	issn = {1931-0145},
	url = {https://doi.org/10.1145/3447556.3447566},
	doi = {10.1145/3447556.3447566},
	abstract = {Deep neural networks (DNNs) have achieved significant performance in various tasks. However, recent studies have shown that DNNs can be easily fooled by small perturbation on the input, called adversarial attacks.},
	journal = {SIGKDD Explor. Newsl.},
	month = {jan},
	pages = {19–34},
	numpages = {16}
}

@article{cora, 
title={Collective Classification in Network Data}, 
volume={29}, url={https://ojs.aaai.org/index.php/aimagazine/article/view/2157}, DOI={10.1609/aimag.v29i3.2157}, abstractNote={Many real-world applications produce networked data such as the world-wide web (hypertext documents connected via hyperlinks), social networks (for example, people connected by friendship links), communication networks (computers connected via communication links) and biological networks (for example, protein interaction networks). A recent focus in machine learning research has been to extend traditional machine learning classification techniques to classify nodes in such networks. In this article, we provide a brief introduction to this area of research and how it has progressed during the past decade. We introduce four of the most widely used inference algorithms for classifying networked data and empirically compare them on both synthetic and real-world data.}, number={3}, journal={AI Magazine}, author={Sen, Prithviraj and Namata, Galileo and Bilgic, Mustafa and Getoor, Lise and Galligher, Brian and Eliassi-Rad, Tina}, year={2008}, month={Sep.}, pages={93} }

@article{KD,
  title={Distilling the Knowledge in a Neural Network},
  author={Geoffrey E. Hinton and Oriol Vinyals and Jeffrey Dean},
  journal={ArXiv},
  year={2015},
  volume={abs/1503.02531}
}

@inproceedings{sgc,
  title={Simplifying graph convolutional networks},
  author={Wu, Felix and Souza, Amauri and Zhang, Tianyi and Fifty, Christopher and Yu, Tao and Weinberger, Kilian},
  booktitle={International conference on machine learning},
  pages={6861--6871},
  year={2019},
  organization={PMLR}
}

@ARTICLE{graphattacksurvey,
  author={Sun, Lichao and Dou, Yingtong and Yang, Carl and Zhang, Kai and Wang, Ji and Yu, Philip S. and He, Lifang and Li, Bo},
  journal={IEEE Transactions on Knowledge and Data Engineering}, 
  title={Adversarial Attack and Defense on Graph Data: A Survey}, 
  year={2022},
  volume={},
  number={},
  pages={1-20},
  doi={10.1109/TKDE.2022.3201243}}

@inproceedings{polblogs,
author = {Adamic, Lada A. and Glance, Natalie},
title = {The Political Blogosphere and the 2004 U.S. Election: Divided They Blog},
year = {2005},
isbn = {1595932151},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/1134271.1134277},
doi = {10.1145/1134271.1134277},
abstract = {In this paper, we study the linking patterns and discussion topics of political bloggers. Our aim is to measure the degree of interaction between liberal and conservative blogs, and to uncover any differences in the structure of the two communities. Specifically, we analyze the posts of 40 "A-list" blogs over the period of two months preceding the U.S. Presidential Election of 2004, to study how often they referred to one another and to quantify the overlap in the topics they discussed, both within the liberal and conservative communities, and also across communities. We also study a single day snapshot of over 1,000 political blogs. This snapshot captures blogrolls (the list of links to other blogs frequently found in sidebars), and presents a more static picture of a broader blogosphere. Most significantly, we find differences in the behavior of liberal and conservative blogs, with conservative blogs linking to each other more frequently and in a denser pattern.},
booktitle = {Proceedings of the 3rd International Workshop on Link Discovery},
pages = {36–43},
numpages = {8},
keywords = {link analysis, political blogs, social networks},
location = {Chicago, Illinois},
series = {LinkKDD '05}
}

@article{deeprobust, title={DeepRobust: a Platform for Adversarial Attacks and Defenses}, volume={35}, url={https://ojs.aaai.org/index.php/AAAI/article/view/18017}, DOI={10.1609/aaai.v35i18.18017}, abstractNote={DeepRobust is a PyTorch platform for generating adversarial examples and building robust machine learning models for different data domains. Users can easily evaluate the attack performance against different defense methods with DeepRobust and get performance analyzing visualization. In this paper, we introduce the functions of DeepRobust with detailed instructions. We believe that DeepRobust is a useful tool to measure deep learning model robustness and to find the suitable countermeasures against adversarial attacks. The platform is kept updated and can be found at https://github.com/DSE-MSU/DeepRobust. More details of instruction can be found in the documentation at https://deeprobust.readthedocs.io/en/latest/.}, number={18}, journal={Proceedings of the AAAI Conference on Artificial Intelligence}, author={Li, Yaxin and Jin, Wei and Xu, Han and Tang, Jiliang}, year={2021}, month={May}, pages={16078-16080} }

@article{LinkPred,
  title={Link prediction based on graph neural networks},
  author={Zhang, Muhan and Chen, Yixin},
  journal={Advances in neural information processing systems},
  volume={31},
  year={2018}
}

@article{community,
  title={Community detection with graph neural networks},
  author={Bruna, Joan and Li, X},
  journal={stat},
  volume={1050},
  pages={27},
  year={2017}
}

@article{homophily,
  title={Birds of a feather: Homophily in social networks},
  author={McPherson, Miller and Smith-Lovin, Lynn and Cook, James M},
  journal={Annual review of sociology},
  pages={415--444},
  year={2001},
  publisher={JSTOR}
}

@inproceedings{aug,
  title={Data Augmentation for Graph Neural Networks},
  author={Zhao, Tong and Liu, Yozen and Neves, Leonardo and Woodford, Oliver and Jiang, Meng and Shah, Neil},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={35},
  number={12},
  pages={11015--11023},
  year={2021}
}

@article{VGAE,
  title={Variational graph auto-encoders},
  author={Kipf, Thomas N and Welling, Max},
  journal={arXiv preprint arXiv:1611.07308},
  year={2016}
}

@inproceedings{localaug,
  title={Local augmentation for graph neural networks},
  author={Liu, Songtao and Ying, Rex and Dong, Hanze and Li, Lanqing and Xu, Tingyang and Rong, Yu and Zhao, Peilin and Huang, Junzhou and Wu, Dinghao},
  booktitle={International Conference on Machine Learning},
  pages={14054--14072},
  year={2022},
  organization={PMLR}
}

@article{MH,
  title={Metropolis-hastings data augmentation for graph neural networks},
  author={Park, Hyeonjin and Lee, Seunghun and Kim, Sihyeon and Park, Jinyoung and Jeong, Jisu and Kim, Kyung-Min and Ha, Jung-Woo and Kim, Hyunwoo J},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={19010--19020},
  year={2021}
}

@article{MHalgorithm,
  title={Monte Carlo sampling methods using Markov chains and their applications},
  author={Hastings, W Keith},
  year={1970},
  publisher={Oxford University Press}
}

@article{NE,
  title={Network enhancement as a general method to denoise weighted biological networks},
  author={Wang, Bo and Pourshafeie, Armin and Zitnik, Marinka and Zhu, Junjie and Bustamante, Carlos D and Batzoglou, Serafim and Leskovec, Jure},
  journal={Nature communications},
  volume={9},
  number={1},
  pages={1--8},
  year={2018},
  publisher={Nature Publishing Group}
}

@ARTICLE{Enet,
  author={Xu, Jiarong and Yang, Yang and Wang, Chunping and Liu, Zongtao and Zhang, Jing and Chen, Lei and Lu, Jiangang},
  journal={IEEE Transactions on Knowledge and Data Engineering}, 
  title={Robust Network Enhancement From Flawed Networks}, 
  year={2022},
  volume={34},
  number={7},
  pages={3507-3520},
  doi={10.1109/TKDE.2020.3025147}}

@article{mincut,
 ISSN = {0364765X, 15265471},
 URL = {http://www.jstor.org/stable/3690374},
 abstract = {The k-cut problem is to find a partition of an edge weighted graph into k nonempty components, such that the total edge weight between components is minimum. This problem is NP-complete for an arbitrary k and its version involving fixing a vertex in each component is NP-hard even for k = 3. We present a polynomial algorithm for k fixed, that runs in $O(n^{k^{2}/2-3k/2+4}T(n,m))$ steps, where T(n, m) is the running time required to find the minimum (s, t)-cut on a graph with n vertices and m edges.},
 author = {Olivier Goldschmidt and Dorit S. Hochbaum},
 journal = {Mathematics of Operations Research},
 number = {1},
 pages = {24--37},
 publisher = {INFORMS},
 title = {A Polynomial Algorithm for the k-Cut Problem for Fixed k},
 urldate = {2022-10-03},
 volume = {19},
 year = {1994}
}










==> improvement_tips.tex <==
\section{Some Tips}
\begin{itemize}
    \item More detailed ablation study should be given, i.e., victim node detection, bilevel structure learning, adaptive threshold.
    \item scalability?
    \item Emphasize the advantage of FocusedCleaner compared with other baselines.
    \item Why use ESR metric?
    \item compare both GASOLINE and GASOLINE-D.
\end{itemize}






























